Exploring Top-Quark Signatures of Heavy Flavor-Violating Scalars at the LHC with Parametrized Neural Networks

In this work, we study flavor-violating scalars (flavons) in a range of large masses that have not been explored previously. We model the interactions with an effective field theory formulation where the flavon is heavier than the top quark. In addition, we assume that the flavon only couples to fermions of the Standard Model in a flavor-changing way. As the flavon couples strongly to top quarks, same-sign and opposite-sign top quark pair signals can be explored in the search for those particles. Using parametrized neural networks, we show that it is possible to probe flavons with masses in the 200-1600 GeV range through their interactions with a top quark plus up and charm quarks for effective couplings of order 10^-2 TeV^-1 at the 14 TeV High-Luminosity LHC.

==> old.tex.tex <==
%\textcolor{magenta}{To enhance our signal efficiency we performed some tunings in our \texttt{run\_card.dat}. We have set \texttt{ebeam1} and \texttt{ebeam2} to 7000 GeV each, emulating the 14 TeV HL LHC. We have also set a minimum $p_T$ for bottom jets and leptons, namely ptb to 30 GeV and ptl to 10 GeV. There is also a window for rapidity, where we set $|\eta| < 2.5$. Finally, we wanted to check for pairs of particles that were not too collimated. For this end we set each minimum $\Delta R$ to 0.5.}

%\textcolor{magenta}{Since we are interested in evading the enormous background from the Drell-Yan process, we also are looking for events with a minimum leptonic invariant mass of 100 GeV. This is more efficiently done directly in the \texttt{run\_card.dat} by setting mmll equals to 100. However, this is only good for pairs of leptons with the same flavor and opposing charges. This is unfortunate in our case since our signal has only the pairs $e^{\pm} e^{\pm}$, $\mu^{\pm} \mu^{\pm}$, and $e^{\pm} \mu^{\mp}$. To circumvent this difficulty, we have also edited the \texttt{setcuts.f} file to cut every lepton pair type. This is the preferred method of selection as we will be able to have a maximum number of events that fulfill our cuts, but this comes at a price of reducing the cross-section displayed at the madgraph.}

%\textcolor{magenta}{After the generation of Monte Carlo events, we select events that survive three types of cut: it must have a lepton pair $e^{\pm} e^{\pm}$, $\mu^{\pm} \mu^{\pm}$, or $e^{\pm} \mu^{\mp}$, it must have two $b$-jets, and the missing energy needs to be at least 20 GeV. This pre-selection left us with 150k events of each mass and each type of signal (final states with two leptons of the same charge or two leptons with opposite charges), and approximately 250-300k of each type of background.}


%\textcolor{magenta}{\subsection{data preparation}}

%\textcolor{magenta}{When we have enough of these events, we train our machine with a few selected flavon masses. The train is successful if the model it generates can predict with high accuracy the mass of some test data that is within the training mass range.}

%\textcolor{magenta}{Once we have simulated all the wanted signal and background events, we start the process of data preparation.}

%\textcolor{magenta}{The first step is to create files containing a mix of a specific flavon mass (with all charge combinations) and all backgrounds. The test data files have approximately 47k events of same charge and 47k of opposite charge events and 35k of combined background events. The train data files are composed of what was left, so approximately 100k of each type of signal events and}


There are several motivations to look for pseudoscalar particles that emerge as pseudo-Nambu-Goldstone bosons (pNGBs) of a spontaneously broken symmetry. One of the most popular is the axion \cite{Weinberg:1977ma,Wilczek:1977pj}, which comes as a solution to the strong CP problem via Peccei-Quinn (PQ) mechanism~\cite{Peccei:1977hh,Peccei:1977ur}. As a result, the axion acquires mass inversely proportional to the spontaneous breaking scale of the U(1)$_{PQ}$ as well as its couplings to Standard Model particles. In the original PQ model, the symmetry-breaking scale $f_a$ had the same order as the electroweak physics, but this model was ruled out due to constraints, for example, from Kaon decays at the National Laboratory for High Energy Physics in Japan (KEK) \cite{Asano:1981nh}, forcing the scale to be very high. However, there are still viable models even when the values of masses and couplings are too small, these models are known as invisible axions models~\cite{Kim:1979if, Shifman:1979if, Dine:1981rt,Zhitnitsky:1980tq}. Although they are the target of several astrophysics experiments, they cannot be probed in colliders, because light candidates are difficult to discriminate from the background. Axion-like particles (ALPs) have some properties similar to the axion, such as couplings suppressed by the global symmetry-breaking scale associated with them. However, in the case of an ALP, there is no direct relation between its mass and its couplings, so the allowed parameter space becomes more susceptible to phenomenological analyses in colliders. This exotic state appears in several possible extensions of the SM ~\cite{PhysRevD95, Ema2017,PhysRevD.81.123530,CHIKASHIGE1981265,GELMINI1981411,PhysRevLett.48.11,PhysRevLett.49.1549,Peter}.

%\textcolor{magenta}{The signal was simulated in three separate categories. Signal 1 is composed of the $pp \to l^{+}l^{+} + v_\ell v_\ell + bb$ processes (and their conjugates) coming either from a double flavon production or from a process where the flavon was exchanged in the $t$-channel. Signal 2 is composed of all the $pp \to  l^+l^- + v_\ell \overline{v_{\ell}} + b \overline{b}$ processes that emerge either from a double flavon production or from a flavon single production (in the $t$- or $s$-channel). Signal 3 is composed of all $pp \to l^{+} l^{-} + v_\ell \overline{v_\ell} + b \overline{b}$, $pp \to l^{+} l^{+} + v_\ell v_\ell + b b$, and their conjugates, arising as decay products of a single flavon production with an accompanying top quark.}


 In this work the new physics is parametrized by a dimension-five effective Lagrangian \cite{GEORGI198673,CHOI1986145} with the hypothesis that the ALP couples only changing the flavor of the Standard Model fermions. This analysis is a sequence of our previous work in \cite{Alves:2023sdf}, where the ALP was lighter than the top quark, but here we assume the ALP to be heavier than the top quark. The Lagrangian is the same as before, it has no relevant couplings to photons, gluons, and electroweak gauge boson pairs and diagonal fermions and we will generically denote these particles by \textit{flavons} independently of the symmetry they are related. If the flavon is heavier than the top quark, it decays primarily to them since the flavon has couplings proportional to the mass of the fermions. Then, the phenomenology changes considerably compared to our last work, where the flavon decays predominantly to tau leptons according to eqs.~\eqref{eq:Lf} and \eqref{eq:condition}. We study the flavon in the production channel of two top quarks up to two non-b-jets including the same sign and opposite sign top quarks in the analysis. Due to the large SM background of $t\bar{t}$ production and Drell-Yan, we use Machine Learning (ML) algorithms to investigate the largest possible parameter space.


\indent Parametrized Neural Networks (pNNs) \cite{pnn1,pnn2} is a new structure of ML classifiers that includes in the feature vector the physical parameters as well. The high energy physics problems usually include in the feature vectors only the kinematic distributions of the final state particles. Today, it is a common practice to test new hypotheses in particle physics since we do not have the best candidate for new physics. Consequently, for each model, we have to scan a large range for the new coupling constants, masses, and so on, unless the model has a specific constraint. However, when using ML classifiers it is necessary to train the model using the signal and background processes you are interested in, but suppose that the new hypothesis predicts the existence of a new massive particle. Since we do not have any clue what this mass could be, it is difficult to decide what is the best training set for the signal. As mentioned in \cite{pnn1}, in the literature, it is possible to find some options, in some of them the collaborations train a single neural network at one intermediate value of the mass and use it for all other mass values \cite{Aad1,PhysRevD.87.072002}, but when this method is applied to other masses the performance of the Neural Network (NN) degrades. Another example is training a model for each mass hypothesis \cite{PhysRevLett.109.071804,201226}, but the mass is a real number, so it is impossible to do it for all values. Furthermore, the interpolation for values outside the trained masses is not allowed since the degradation of the performance is not defined for them. In addition, it can be computationally expensive to train and adjust the hyperparameters for each mass. It is in this context that the pNNs emerge: if the particle mass and any other parameters are included in the feature vector used in the simulation, the pNNs might be able to interpolate the algorithm for other masses not used in the training set. In other words,  we'll have a unique classifier able to discriminate all mass hypotheses. There are some important points we have to take care of, one of them is that smooth interpolation can be done using neural networks, but tree-based methods such as Boosting Decision Trees (BDTs) or other similar might not be possible, since we need a parametric model. Another point is that the extrapolation for masses outside the range of the training set might not work in principle, since the common ML algorithms are only able to interpolate.

To check the validity of this method, we chose three signal channels and their associated backgrounds to train. With a handful of high-level variables as our data parametrization, we trained our pNN for five evenly spaced flavon masses in the range [200, 1400] GeV. The test was performed for each mass in the same range as the train but with a spacing of 100 GeV between subsequent masses. The pNN was able to give a high accuracy for this test battery, with the precision increasing as the flavon mass was increased.



\section{SIGNAL AND BACKGROUND SIMULATIONS}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.45\linewidth]{xsec.pdf}
    \caption{Production cross sections of all three modes considered in this work.}
    \label{fig:xsec}
\end{figure}


\begin{table}
\scalefont{1}
\begin{tabular}{c c c}
\hline
Backgrounds & & $\sigma$ (pb) \\ 
\hline\hline
Drell-Yan    & \;\;\;\;\;\;\;\;\;\;\;\; & 331.11 \\ 
\hline
$t\bar{t}$   &  \;\;\;\;\;\;\;\;\;\;\;\;  & 7.31 \\
\hline
$tW$         &  \;\;\;\;\;\;\;\;\;\;\;\;  & 0.82 \\
\hline
\end{tabular}
\centering
\caption{Cross-sections for the backgrounds in picobarns after the minimal selection.}
\label{tab:double}
\end{table}


%\textcolor{magenta}{To enhance our signal efficiency we performed some tunings in our \texttt{run\_card.dat}. We have set \texttt{ebeam1} and \texttt{ebeam2} to 7000 GeV each, emulating the 14 TeV HL LHC. We have also set a minimum $p_T$ for bottom jets and leptons, namely ptb to 30 GeV and ptl to 10 GeV. There is also a window for rapidity, where we set $|\eta| < 2.5$. Finally, we wanted to check for pairs of particles that were not too collimated. For this end we set each minimum $\Delta R$ to 0.5.}

%\textcolor{magenta}{Since we are interested in evading the enormous background from the Drell-Yan process, we also are looking for events with a minimum leptonic invariant mass of 100 GeV. This is more efficiently done directly in the \texttt{run\_card.dat} by setting mmll equals to 100. However, this is only good for pairs of leptons with the same flavor and opposing charges. This is unfortunate in our case since our signal has only the pairs $e^{\pm} e^{\pm}$, $\mu^{\pm} \mu^{\pm}$, and $e^{\pm} \mu^{\mp}$. To circumvent this difficulty, we have also edited the \texttt{setcuts.f} file to cut every lepton pair type. This is the preferred method of selection as we will be able to have a maximum number of events that fulfill our cuts, but this comes at a price of reducing the cross-section displayed at the madgraph.}

%\textcolor{magenta}{After the generation of Monte Carlo events, we select events that survive three types of cut: it must have a lepton pair $e^{\pm} e^{\pm}$, $\mu^{\pm} \mu^{\pm}$, or $e^{\pm} \mu^{\mp}$, it must have two $b$-jets, and the missing energy needs to be at least 20 GeV. This pre-selection left us with 150k events of each mass and each type of signal (final states with two leptons of the same charge or two leptons with opposite charges), and approximately 250-300k of each type of background.}


%\textcolor{magenta}{\subsection{data preparation}}

%\textcolor{magenta}{When we have enough of these events, we train our machine with a few selected flavon masses. The train is successful if the model it generates can predict with high accuracy the mass of some test data that is within the training mass range.}

%\textcolor{magenta}{Once we have simulated all the wanted signal and background events, we start the process of data preparation.}

%\textcolor{magenta}{The first step is to create files containing a mix of a specific flavon mass (with all charge combinations) and all backgrounds. The test data files have approximately 47k events of same charge and 47k of opposite charge events and 35k of combined background events. The train data files are composed of what was left, so approximately 100k of each type of signal events and}

We simulated signals and backgrounds in leading order at the 14 TeV LHC with \texttt{MadGraph5}~\cite{Alwall:2014hca, Frederix:2018nkq} using the \texttt{UFO}~\cite{Degrande:2011ua} files generated by \texttt{FeynRules}~\cite{Alloul:2013bka} where we implemented our effective model.  The parton shower and detector simulations were performed in the default settings of \texttt{PYTHIA 8.3} \cite{Bierlich:2022pfr} and \texttt{Delphes3}~\cite{deFavereau:2013fsa}, respectively. The signal we consider involves the production of 2 top quarks with the same or opposite signs, and up to 2 non-$b$ jets. To achieve this we consider the following signal processes: the flavon in the $t$ channel (0 non-$b$ jet),  as well as the single (1 non-$b$ jet) and double production of flavons (2 non-$b$ jets) as shown in Fig. \ref{fig:prod}. 

%\textcolor{magenta}{The signal was simulated in three separate categories. Signal 1 is composed of the $pp \to l^{+}l^{+} + v_\ell v_\ell + bb$ processes (and their conjugates) coming either from a double flavon production or from a process where the flavon was exchanged in the $t$-channel. Signal 2 is composed of all the $pp \to  l^+l^- + v_\ell \overline{v_{\ell}} + b \overline{b}$ processes that emerge either from a double flavon production or from a flavon single production (in the $t$- or $s$-channel). Signal 3 is composed of all $pp \to l^{+} l^{-} + v_\ell \overline{v_\ell} + b \overline{b}$, $pp \to l^{+} l^{+} + v_\ell v_\ell + b b$, and their conjugates, arising as decay products of a single flavon production with an accompanying top quark.}

\begin{figure}
    \centering
    \input{qg_at_T} \input{qg_at_S}  
    \input{qq_aa} \input{at}
    \caption{Concerning the upper Feynman diagrams, the left and middle ones refer to the single production of flavons, while the upper right refers to the double production of flavons. The lower diagram is the leading order diagram in which the flavon is in t-channel.}
    \label{fig:prod}
\end{figure}
\indent In the effective model we are working on, the coupling constant of the flavon to fermions is proportional to the mass of the fermions. As a result, almost 100\% of its branching ratio is to top quark + jet. To take some advantage of this fact, we only consider reactions where the flavon decays to them (or their antiparticles), namely, $a \rightarrow t \bar{q}$ where $q=u,c$. Then, in the production channel, we always have 2 top quarks and up to 2 non-$b$ jets. The top quark branching ratio is dominated by $Wb$, so its branching ratio is determined by the $W$ branching ratio. For the $W$ boson we decay it to $W^+ \rightarrow \ell^+ + \nu_{\ell}$, with $\ell = e,\mu$. Table \ref{tab:double} summarizes the signal and background processes.


\begin{table}
%\scalefont{0.8}
\begin{tabular}{c c c}
\hline
Signals & &  \\ 
\hline\hline
0 non-bjet    & \;\;\;\;\;\;\;\;\;\;\;\;   & same sign: $
pp \rightarrow tt\;(\bar{t}\bar{t}) \rightarrow \ell^+ \ell^+ \nu_{\ell} \nu_{\ell} bb  \; (\ell^- \ell^- \bar{\nu}_{\ell} \bar{\nu}_{\ell} \bar{b}\bar{b})$    \\ 
 & & opposite sign: $pp \rightarrow t\bar{t} \rightarrow \ell^+ \ell^- \nu_{\ell} \bar{\nu}_{\ell} b\bar{b}  $ \\
\hline
1 non-bjet   & \;\;\;\;\;\;\;\;\;\;\;\;    & same sign: $pp \rightarrow at (a\bar{t}) \rightarrow \ell^+ \ell^+ \nu_{\ell} \nu_{\ell} bbj  \; (\ell^- \ell^- \bar{\nu}_{\ell} \bar{\nu}_{\ell} \bar{b}\bar{b}j) $  \\
 &  &  opposite sign: $pp \rightarrow at(a\bar{t}) \rightarrow \ell^+ \ell^- \nu_{\ell} \bar{\nu}_{\ell} b\bar{b}j$ \\
\hline
2 non-bjet         &  \;\;\;\;\;\;\;\;\;\;\;\;  & same sign:  $pp \rightarrow aa \rightarrow \ell^+ \ell^+ \nu_{\ell} \nu_{\ell} bbjj  \; (\ell^- \ell^- \bar{\nu}_{\ell} \bar{\nu}_{\ell} \bar{b}\bar{b}jj) $  \\
 &    & opposite sign: $pp \rightarrow aa \rightarrow \ell^+ \ell^- \nu_{\ell} \bar{\nu}_{\ell} b\bar{b}jj $\\ 
\hline
Backgrounds & &   \\
\hline
$t\bar{t}$ & & $pp \rightarrow t\bar{t} \rightarrow \ell^+ \ell^- \nu_{\ell} \bar{\nu}_{\ell} b\bar{b} $ \\
\hline
Drell-Yan & & $pp \rightarrow \ell^+ \ell^-$ up to two non-bjets\\
\hline
single top  & & $pp \rightarrow tW^- (\bar{t}W^+) \rightarrow \ell^+ \ell^- \nu_{\ell} \bar{\nu}_{\ell} b(\bar{b}) $ \\
\hline
\end{tabular}
\centering
\caption{Summary of the process considered in this work, the three first ones refer to the signal up to two non-b jets and the last three refer to the backgrounds.}
\label{tab:double}
\end{table}

\indent One possibility would be to consider only an exotic final state that comes from the production of same-sign top quarks. However, due to detector efficiencies, if some of the leptons are not detected, the NN can only discriminate signal events from the background by looking at the kinematical distributions. As you can see in Figure~\ref{fig:distros}, the distributions are similar, because of that we decided to add the signal process of top quarks of opposite sign, since the significance considering only the exotic final state cannot be the square root of the signal events, then adding more signal we increase the significance.

\section{analysis}

\indent Before we pass the data generated by Monte Carlo in the pNN we did a minimal selection and constructed high-level variables. We chose events that contained exactly two $\ell = e, \mu$ with any electric charge, at least one $b$ quark, where the particles respected the following kinematic thresholds: 
\begin{equation}
p_{T_{\ell}} > 10 \,\mbox{GeV}\,, \quad  p_{T_{j,b}} > 20 \,\mbox{GeV}\,, \quad \left|\eta_{\ell,j}\right| < 2.5 \,, \quad M_{\ell_1 \ell_2} > 100 \,, \quad \slashed{E}_T > 20 \, \si{GeV} \,,
\end{equation}
where $\ell_{1,2}$ are the leptons ordered by decreasing transverse momenta. This set of cuts has an efficiency of approximately 8\% on the signal and 12.5\% on the backgrounds. After this minimal selection, the cross sections for the signals and backgrounds are displayed in Figure \ref{fig:xsec} and Table \ref{tab:double}, respectively.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.45\linewidth]{xsec.pdf}
    \caption{Production cross sections of all three modes considered in this work.}
    \label{fig:xsec}
\end{figure}

\begin{table}
\scalefont{1}
\begin{tabular}{c c c}
\hline
Backgrounds & & $\sigma$ (pb) \\ 
\hline\hline
Drell-Yan    & \;\;\;\;\;\;\;\;\;\;\;\; & 331.11 \\ 
\hline
$t\bar{t}$   &  \;\;\;\;\;\;\;\;\;\;\;\;  & 7.31 \\
\hline
$tW$         &  \;\;\;\;\;\;\;\;\;\;\;\;  & 0.82 \\
\hline
\end{tabular}
\centering
\caption{Cross-sections for the backgrounds in picobarns after the minimal selection.}
\label{tab:double}
\end{table}
%
\indent In what respects the high-level variables, because of the large number of particles in the final state we can construct a large number of distributions combining them. However, if you increase the number of distributions too much this can have a large computational cost and it may also reduce the power of discernment of the neural network. For the problem in question, the set of variables displayed in Table \ref{tab:double2} is sufficient to observe the signal.
%
\begin{table}
\scalefont{1}
\begin{tabular}{c}
\hline
Variables   \\ 
\hline\hline
$p_{T_{\ell_{1, 2}}}$, $p_{T_{b_{1, 2}}}$, $p_{T_{j_{1}}}$, $p_{T_{\mathrm{miss}}}$, $E_{\ell_{1,2}}$, $E_{b_{1, 2}}$ \\
\hline
$\eta_{\ell_{1,2}}$, $\eta_{b_{1,2}}$, $\eta_{j_1}$, $m_{\ell_1 \ell_2}$, $m_{\ell_1 b_1}$, $m_{\ell_1 b_2}$, $m_{\ell_1 j_1}$, $m_{\ell_2 b_1}$, $m_{\ell_2 b_2}$, $m_{b_1 b_2}$, $m_T$ \\
\hline
$\Delta R_{\ell_1 \ell_2}$, $\Delta R_{\ell_1 b_1}$, $\Delta R_{\ell_1 b_2}$, $\Delta R_{\ell_1 j_1}$, $\Delta R_{\ell_2 b_1}$, $\Delta R_{\ell_2 b_2}$, $\Delta R_{b_1 b_2}$, $\Delta\phi_{1234}$ \\
\hline
$\mu^+$, $\mu^-$, $e^+$, $e^-$, $b$-jets, jets, $m_a$ \\
\hline
\end{tabular}
\centering
\caption{Complete list of all variables considered for the analysis in the pNN. Here, $p_T$ stands for the transverse momentum, $E$ the energy, $\eta$ the pseudorapidity, $m_T$ the transverse mass, $\Delta R$ invariant angular distance, $\mu^+$, $\mu^-$, $e^+$, $e^-$, $b$-jets are the number of these particles in the final state, $m_a$ the flavon mass and $\Delta \phi$ the difference between the azimuthal angle of the particles. The numerical index orders the particles in the same class ($\ell$, $b$, and $j$) by $p_T$.}
\label{tab:double2}
\end{table}

The main advantage of using pNNs is the possibility of including the parameter that will be interpolated. In this case, we included the flavon mass in the feature vector. There is one point here: we do not have an analogous mass for the background, since we use $m_a$ to denote the flavon mass. The way out of this is to assign to each background event a random value among the grid previously chosen for the flavon mass. There are two options to do it, one is to use a discrete distribution and the other a continuous distribution, but according to \cite{pnn2} the continuous distribution easily overfits the result.

Regarding training, we balance the number of signal and background events used in it, because according to Ref. \cite{pnn2} this imbalance might decrease the performance of the algorithm. The pNN was trained with the following set of masses [200,500,800,1100,1400], so to keep this balanced the sum of the signal events must be equal to the sum of the background events. As usual, we use the MinMax function to scale the data as well as the standardization of the data.

The training was done with 270000 events divided to contain the same number of signal and background events. To attest to the model's robustness, we performed a 10-fold cross-validation and found a mean training accuracy of 89\%.

To optimize the model as much as we can, the hyperparameter search was performed using the Hyperopt package \cite{hyperopt}, which uses a Bayesian optimization method called Tree of Parzen Estimators \cite{bergs} to find the best set of hyperparameters. In this set, we consider the learning rate, batch size, number of Hidden layers, different activation functions, dropout, and the number of neurons. The best set we found is shown in Table \ref{tab:hyperparam}:
% 
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}
    \begin{tabular}{@{}cccccc@{}}
    \hline
    hidden layers & neurons & activation & drop-out & learning rate & batch size \\ \hline \hline
    3                      & 80               & elu                          & 0.265             & 0.00156                & 80                  \\ \hline
    \end{tabular}

\centering
\caption{Complete list of all variables considered for the analysis in the pNN.}
\label{tab:hyperparam}
\end{table}

\indent To improve the learning rate during the training we use Adam \cite{kingma2017adam} and learning rate scheduler [...]. To avoid overfitting it was also used the early stopping [...].
%
The loss used in this project was the binary cross-entropy, in addition, we set the number of epochs to two hundred. The data set is split into three sets: training set, validation set, and test set. The model looks only at the training set when it is actively training and deciding how to change its weights. After every training epoch, we check how the model is doing by looking at the training loss and the loss of the validation set. It's important to remember that the validation set nor the test set is used in any part of the training. Since the model does not use the validation set to train the model it can be used to see if there is overfitting. \\
%
\indent In practice, the main property of pNNs is not to discriminate the mixed signal from the background but the goal is how each mass within the range of [200,1400] GeV is discriminated from the background even when the mass of the particle is outside the masses used in the training set. The Figure~\ref{fig:mass-inside} shows the distribution of the signal (red) and background (blue) events as a function of the classifier output.

\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{dnn-200.pdf}
    \includegraphics[width=0.45\linewidth]{dnn-1100.pdf}
    \includegraphics[width=0.45\linewidth]{dnn-300.pdf}
    \includegraphics[width=0.45\linewidth]{dnn-1000.pdf}
    \caption{The figures on the left show the distribution of the signal events (red) and background events (blue) in terms of the score function for the masses inside the training set. On the right, it shows their confusion matrix.}
    \label{fig:mass-inside}
\end{figure}


It is clear from Figure \ref{fig:mass-inside} that the lighter flavon hypothesis is more difficult to discriminate from the background as expected according to the distributions in Figure \ref{fig:distros}. The pictures on the right show the confusion matrix, the diagonal elements correspond to the correct classifications, while the non-diagonal elements refer to the wrong classifications. The upper off-diagonal element of the matrix corresponds to signal events incorrectly classified as background events and the lower off-diagonal element to background events classified as signal events. Analyzing the non-diagonal elements of the matrix we conclude that both of them have similar power of classification.

%\indent  In the figure (\ref{fig:mass-outside}) we can finally see the performance of the pNN in masses outside the training set, if we compare the masses of 200 with 300 GeV and 1100 with 1000 GeV, it's clear that the performance is similar for both masses. However, remember that the masses [200,1100] were used in the training, while the masses [300,1000] were not used. Of course, each mass has its kinematic distributions and the performance won't be the same, but the main point is that the performance does not degrade for masses outside the training set. 

\begin{figure}
    \centering    \includegraphics[width=0.45\linewidth]{roc.pdf}
    \caption{Fraction of surviving signal $\varepsilon_S$ versus the fraction of surviving background $\varepsilon_B$ as functions of the score threshold.}
    \label{fig:roc}
\end{figure}

In Figure \ref{fig:roc} we see the algorithm performance for each test mass. $\varepsilon_S$ and $\varepsilon_B$ are the fractions of signal and background events that survive for a given threshold score cut. It is possible to see that the peak performance occurs at around $m_a = 1000$ GeV. After this peak, the performance decreases slightly for each subsequent mass.

%\begin{figure}[H]
%    \centering
%    \includegraphics[scale=0.5]{pics/300_scores.pdf}
%     \includegraphics[scale=0.5]{pics/300_cmatrix.pdf}
         %\includegraphics[scale=0.5]{pics/900_scores.pdf}
     %\includegraphics[scale=0.5]{pics/900_cmatrix.pdf}
%          \includegraphics[scale=0.5]{pics/1500_scores.pdf}
%     \includegraphics[scale=0.5]{pics/1500_cmatrix.pdf}
%    \caption{The figures on the left shows the distribution of the signal events (red) and background events (blue) in terms of the score function for the masses outside the training set. On the right it's showed their confusion matrix.}
%    \label{fig:mass-outside}
%\end{figure}
%\vspace{-0.2cm}



In the next section we present an estimate of the exclusion and discovery limits for a flavon heavier than the top quark in the 14 TeV LHC for luminosities of 3000 and 4000 $fb^{-1}$. To extract the limits, we used a modified version of the Asimov estimate for the statistical significance~\cite{Cowan_2011}

\begin{equation}{
    Z(S,B,\varepsilon) = 
    \begin{cases}
        \sqrt{S} \,, \quad &\text{when } \varepsilon=0  \text{ and } B=0 \\
        \sqrt{-2S+2(S+B) \ln \left( 1 + \frac{S}{B} \right)}  \,, \quad &\text{when }  \varepsilon =0 \text{ and } 0<B<500 S\\
        \sqrt{2(S+B) \ln\left( \frac{(S+B)(1+\varepsilon)}{B + (S+B) \varepsilon} \right)  -2 \frac{B}{\varepsilon} \ln \left( 1 + \frac{S \varepsilon}{B + B \varepsilon}\right)}   \,, \quad &\text{when }  \varepsilon \neq 0 \text{ and } 0<B<500S \\
        \frac{S}{\sqrt{B(1+\varepsilon)}}  \,, &\text{else}
    \end{cases}}
\end{equation}
where $S$ and $B$ are, respectively, the numbers of surviving signal and background events after the cuts are performed, and $\varepsilon$ is the estimated systematic uncertainty of the total background rate, related to the uncertainty in $B$ by $\sigma_b^2 = \varepsilon B$.

To guarantee the Asimov function is computationally well-behaved in all possible regimes when $\varepsilon \in [0,1)$, $S \in [1, \infty)$, and $B \in [0, \infty)$, we perform power expansions and keep only the leading term. This is a needed step since the function displays bad behavior when $B/S \gg 500$. When this limit is extrapolated, we use instead the well-known approximation $S/\sqrt{B(1+\varepsilon)}$ that reduces to $S/\sqrt{B}$ when $\varepsilon \to 0$. In the case where $B=\varepsilon=0$, the Asimov statistic goes to infinity, so we use instead the $\sqrt{S}$ estimation.

\section{RESULTS}

\indent The figures below display the exclusion and discovery limits as a function of the ratio of cutoff and the Wilson coefficient in terms of the flavon mass for four systematic error scenarios:

%\begin{figure}[H]
%    \centering
%    \includegraphics[scale=0.5]{pics/3.pdf}
%    \caption{Caption}
%    \label{fig:3}
%\end{figure}

\begin{figure}
    \centering    \includegraphics[width=0.45\linewidth]{limit-5.pdf}
\includegraphics[width=0.45\linewidth]{limit-50.pdf}
    \caption{Benchmark limits for the pNN under different percentages of systematic errors. Each curve is an interpolation of the training data results that were calculated in an evenly spaced grid with a spacing of 100 GeV.}
    \label{fig:3-inv}
\end{figure}

%\begin{figure}[H]
%    \centering
%    \includegraphics[scale=0.5]{pics/4.pdf}
%    \caption{Caption}
%    \label{fig:4}
%\end{figure}

\indent First of all, the region $m_a > \Lambda$ refers to a validity limit for the EFT. We can observe that for both luminosities it is possible to probe cutoffs of the order 0.4 TeV$^{-1}$ depending on the mass, in addition, the exclusion/discovery region reaches flavon masses of around 1.2 TeV with the channels we proposed. Due to the large cross sections of the background events, despite the Drell-Yan background being reducible, it would be very unlike that with rectangular cuts we could observe the flavon in this channel, this shows in one more example the crucial importance of neural networks. Furthermore, the pNNs come as an important tool to discriminate signal from background events with a unique model without degrading performance outside the masses used in the training set, \textcolor{red}{this can be viewed in plots with the performance smoothly decreasing}. To conclude, the effect of systematic error up to 20\% is negligible in this analysis.





\section{CONCLUSIONS}

==> pics/drell-yan_plus_jets.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]
    \begin{feynman}
        \vertex (a1) {\(q\)};
        \vertex[below right = 0.5cm and 2cm of a1] (a2);
        \vertex[right =1cm of a2] (a3);
        \vertex[above right = 0.5cm and 1cm of a3] (au) {\(\ell^{-}\)};
        \vertex[below right = 0.5cm and 1cm of a3] (ad) {\(\ell^{+}\)};
        \vertex[below =1.2cm of a2] (b2);
        \vertex[below right = 0.5cm and 2cm of b2] (b3) {\(q\)};
        \vertex[below =1.2cm of b2] (c2);
        \vertex[below left = 0.5cm and 2cm of c2] (c1) {\(g\)};
        \vertex[below right = 0.5cm and 2cm of c2] (c3) {\(g\)};
        \diagram*{
            (a1) -- [fermion] (a2),
            (a2) -- [boson, edge label=\(\gamma\)] (a3),
            (a3) -- [fermion] (au),
            (a3) -- [anti fermion] (ad),
            (a2) -- [fermion, edge label'=\(q\)] (b2),
            (b2) -- [fermion] (b3),
            (b2) -- [gluon, edge label'=\(g\)] (c2),
            (c1) -- [gluon] (c2),
            (c2) -- [gluon] (c3),
        };
    \end{feynman}
\end{tikzpicture}

==> pics/test.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]
    \begin{feynman}
        \vertex (a1) {\(q\)};
        \vertex[below right = 1cm and 3cm of a1] (a2);
        \vertex[above right = 0.5cm and 1cm of a2] (a3);
        \vertex[above right = 0.5cm and 1cm of a3] (a4u);
        \vertex[below right = 0.5cm and 1cm of a3] (a4d);
        \vertex[above right = 0.5cm and 1cm of a4d] (a5u);
        \vertex[below right = 0.5cm and 1cm of a4d] (a5d);
        \vertex[below = of a2] (b2);
        \vertex[below left = 1cm and 3cm of b2] (b1);
        \vertex[below right = 0.5cm and 1cm of b2] (b3);
        \vertex[above right = 0.5cm and 1cm of b3] (b4u);
        \vertex[below right = 0.5cm and 1cm of b3] (b4d);
        \vertex[above right = 0.5cm and 1cm of b4u] (b5u);
        \vertex[below right = 0.5cm and 1cm of b4u] (b5d);
        \diagram*{
            (a1) -- [fermion] (a2),
            (a2) -- [boson, edge label=\(\gamma\)] (a3),
            (a2) -- [boson] (b2);
            (b1) -- [fermion] (b2);
            (b2) -- [fermion] (b3);
            (a3) -- [fermion] (a4u);
            (a3) -- [boson] (a4d);
            (b3) -- [boson] (b4u);
            (b3) -- [fermion] (b4d);
            (b4u) -- [boson] (b5u);
            (b4u) -- [fermion] (b5d);
            (a4d) -- [scalar] (a5u);
            (a4d) -- [scalar] (a5d);
        };
    \end{feynman}
\end{tikzpicture}

==> pics/ttbar.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]
    \begin{feynman}
        \vertex (a1) {\(g\)};
        \vertex[below right = 1.2cm and 2cm of a1] (b2);
        \vertex[right = of b2] (b3);
        \vertex[above right = 1.2cm and 1cm of b3] (a4);
        \vertex[above right = 0.4cm and 2cm of a4] (a5u) {\(b\)};
        \vertex[below right = 0.5cm and 1cm of a4] (a5d);
        \vertex[below left = 1.2cm and 2cm of b2] (c1) {\(g\)};
        \vertex[below right = 1.2cm and 1cm of b3] (c4);
        \vertex[above right = 0.5cm and 1cm of c4] (c5u);
        \vertex[below right = 0.4cm and 2cm of c4] (c5d) {\(\bar{b}\)};
        \vertex[above right = 0.2cm and 1cm of a5d] (a6u) {\(\ell^{-}\)};
        \vertex[below right = 0.2cm and 1cm of a5d] (a6d) {\(\bar{\nu_\ell}\)};
        \vertex[above right = 0.2cm and 1cm of c5u] (c6u) {\(\nu_\ell\)};
        \vertex[below right = 0.2cm and 1cm of c5u] (c6d) {\(\ell^{+}\)};
        \diagram*{
            (a1) -- [gluon] (b2),
            (b2) -- [gluon, edge label=\(g\)] (b3),
            (b3) -- [fermion, edge label=\(t\)] (a4),
            (c1) -- [gluon] (b2),
            (b3) -- [anti fermion, edge label'=\(\bar{t}\)] (c4),
            (a4) -- [boson] (a5d),
            (a4) -- [fermion] (a5u),
            (c4) -- [boson] (c5u),
            (c4) -- [anti fermion] (c5d),
            (a5d) -- [fermion] (a6u),
            (a5d) -- [anti fermion] (a6d),
            (c5u) -- [fermion] (c6u),
            (c5u) -- [anti fermion] (c6d),
        };
    \end{feynman}
\end{tikzpicture}

==> qg_at_S.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]
    \begin{feynman}
        \vertex (b2);
        \vertex [above left=of b2] (a1) {\(q\)};
        \vertex [below left=of b2] (c1) {\(g\)};
        \vertex [right=of b2] (b3);
        \vertex [above right=of b3] (a4) {\(a\)};
        \vertex [below right=of b3] (c4) {\(t\)};
        \diagram* {
            (a1) -- [fermion] (b2) -- [gluon] (c1),
            (b2) -- [fermion, edge label=\(q\)] (b3),
            (a4) -- [scalar] (b3) -- [fermion] (c4),
        };
    \end{feynman}
\end{tikzpicture}

==> setcuts.tex <==
      do i=nincoming+1,nexternal-1
         do j=i+1,nexternal
            s_min(j,i)=0.0d0**2
            s_max(j,i)=-1
            if(do_cuts(i).and.do_cuts(j)) then
               if(is_a_j(i).and.is_a_j(j)) s_min(j,i)=mmjj*dabs(mmjj)   
               if(is_a_a(i).and.is_a_a(j)) s_min(j,i)=mmaa*dabs(mmaa)  
               if( is_a_b(i).and.is_a_b(j) ) s_min(j,i)=mmbb*dabs(mmbb)     
               if((is_a_l(i).and.is_a_l(j)).and.
     &            (abs(idup(i,1,iproc)).eq.abs(idup(j,1,iproc))).and.
     &            (idup(i,1,iproc)*idup(j,1,iproc).lt.0)) 
     &            s_min(j,i)=mmll*dabs(mmll)  !only on l+l- pairs (same flavour) 

               if(is_a_j(i).and.is_a_j(j)) s_max(j,i)=mmjjmax*dabs(mmjjmax)   
               if(is_a_a(i).and.is_a_a(j)) s_max(j,i)=mmaamax*dabs(mmaamax)  
               if( is_a_b(i).and.is_a_b(j) ) s_max(j,i)=mmbbmax*dabs(mmbbmax)     
               if((is_a_l(i).and.is_a_l(j)).and.
     &            (abs(idup(i,1,iproc)).eq.abs(idup(j,1,iproc))).and.
     &            (idup(i,1,iproc)*idup(j,1,iproc).lt.0)) 
     &            s_max(j,i)=mmllmax*dabs(mmllmax)  !only on l+l- pairs (same flavour)
            endif
         enddo
      enddo
